Segmenting white matter hyperintensities on isotropic three-dimensional Fluid Attenuated Inversion Recovery magnetic resonance images: Assessing deep learning tools on norwegian imaging database

Automated segmentation of white matter hyperintensities (WMHs) is an essential step in neuroimaging analysis of Magnetic Resonance Imaging (MRI). Fluid Attenuated Inversion Recovery (FLAIR-weighted) is an MRI contrast that is particularly useful to visualize and quantify WMHs, a hallmark of cerebral small vessel disease and Alzheimer's disease (AD). Clinical MRI protocols migrate to a three-dimensional (3D) FLAIR-weighted acquisition to enable high spatial resolution in all three voxel dimensions. The current study details the deployment of deep learning tools to enable automated WMH segmentation and characterization from 3D FLAIR-weighted images acquired as part of a national AD imaging initiative. Among 441 participants (194 male, mean age: (64.91 +/- 9.32) years) from the DDI study, two in-house networks were trained and validated across five national collection sites. Three models were tested on a held-out subset of the internal data from the 441 participants and an external dataset with 29 cases from an international collaborator. These test sets were evaluated independently. Five established WMH performance metrics were used for comparison against ground truth human-in-the-loop segmentation. Results of the three networks tested, the 3D nnU-Net had the best performance with an average dice similarity coefficient score of 0.76 +/- 0.16, performing better than both the in-house developed 2.5D model and the SOTA Deep Bayesian network. With the increasing use of 3D FLAIR-weighted images in MRI protocols, our results suggest that WMH segmentation models can be trained on 3D data and yield WMH segmentation performance that is comparable to or better than state-of-the-art without the need for including T1-weighted image series.

==> section_files/figures.tex <==


% \begin{figure}[htp]
% \centering
% \includegraphics[width=1\textwidth]{article_images/Figure1_color.jpg}
% \caption{Distribution of total WMH volume per subject in the multi-center internal dataset. The median and interquartile range of the total WMH volume was  2.98(1.29-5.83) mL and the total range (0.11-78.26) mL.}
% \label{fig:Figure1}
% \end{figure}

% \begin{figure}[htp]
%     \centering
%     \includegraphics[width=1\textwidth]{article_images/Figure2_color.jpg}
%     \caption{ Boxplot of the internal test data (n = 60) performance metrics. The 3D nnU-Net is favorable for all metrics, giving the best means for all metrics with a p-value < 0.001 compared to the other models. The p-value legends are: ns: 0.05 < p <= 1.00, *: 0.01 < p <= 0.05,  **: 0.001 < p <= 0.01, ***: 0.0001 < p <= 0.001, ****: p <= 0.0001.
%     }
%     \label{fig:Figure2}
%     \end{figure}
    

% \begin{figure}[htp]
% \centering
% \includegraphics[width=1\textwidth]{article_images/Figure3_color.jpg}
% \caption{Boxplot of the external test data (n = 29) performance metrics.The p-value legends are: ns: 0.05 < p <= 1.00 *: 0.01 < p <= 0.05 
% **: 0.001 < p <= 0.01 ***: 0.0001 < p <= 0.001 ****: p <= 0.0001.}
% \label{fig:Figure3}
% \end{figure}


% \begin{figure}[htp]
%     \centering
%     \includegraphics[width=1\textwidth]{article_images/Figure4_color.jpg}
%     \caption{Example 1 of segmentations on internal test data for all three models overlayed onto FLAIR-weighted-weighted images. TP is a true positive, FP is a false positive and FN is a false negative.}
%     \label{fig:Figure4}
%     \end{figure}


    
% \begin{figure}[htp]
%     \centering
%     \includegraphics[width=1\textwidth]{article_images/Figure5_color.jpg}
%     \caption{Example 2 segmentations on the internal test data for all three models overlayed on FLAIR-weighted.TP is a true positive, FP is a false positive and FN is a false negative.}
%     \label{fig:Figure5}
%     \end{figure}


% \begin{figure}[htp]
% \centering
% \includegraphics[width=1\textwidth]{article_images/Figure6_color.jpg}
% \caption{Example segmentations of external test data for all three models overlayed on FLAIR-weighted. TP is a true positive, FP is a false positive and FN is a false negative.}
% \label{fig:Figure6}
% \end{figure}


% \begin{figure}[htp]
% \centering
% \includegraphics[width=1\textwidth]{article_images/Figure7_color.jpg}
% \caption{Histogram of the FLAIR-weighted MRI image intensity means and intensity entropy across all image volumes in their respective data sets. Note the large deviation the distributions for the external test data compared to the training and internal test data.}
% \label{fig:Figure7}
% \end{figure}

==> section_files/tables.tex <==

 
%  \begin{table*}[htb]
%     \caption{Dataset information for the internal dataset. The external dataset uses Prisma only with the same parameters.}
%     	\begin{adjustwidth}{-2.6cm}{}
% 	% \resizebox{0.9\textwidth}{!}{
%     \begin{tabular}{l|l|l|l|l|l|l|l}
%         Institution        & Model &   Software &  \parbox[t]{1cm}{Field\\Strength} & \parbox[t]{1cm}{Repetition\\ Time (msec)}& \parbox[t]{1cm}{Echo\\ Time (msec)}& \parbox[t]{1cm}{Flip\\ Angle (deg)} & \parbox[t]{1cm}{Resolution \\(x,y,z) (mm)} \\\hline
%         Institution 1 & Avanto &syngo\_MR\_B19 & 1.5 & 1700 & 2.42 & 15 & (1.2,1.05,1.05) \\
%         Institution 2 & Avanto &syngo\_MR\_B19 & 1.5 & 1700 & 2.42 & 15 & (1.2, 1.04, [1.0,1.04]) \\
%         Institution 3 & Avanto &syngo\_MR\_B19 & 1.5 & 1700 & 2.42 & 15 & (1.2,1.05,1.05) \\
%         Institution 4 & Avanto &syngo\_MR\_B19 & 1.5 & 1180 & 4.36 & 15 & (1.0, 1.0, 1.0) \\
%         Institution 5 & Ingenia &[5.1.7,5.3.0.3] & 3.0 & [4.47, 4.91] & [2.218, 2.431] & 8 & ([1.0, 1.2], 1.2, 1) \\
%         Institution 6 & Prisma & syngo\_MR\_E11 & 3.0 & 2200 & 1.47 & 8 & (1.0, 1.0, 1.0)\\
%         Institution 7 & Skyra & syngo\_MR\_E11 & 3.0 & 2300.0 & 2.98 & 9 & (1.2, 1.0, 1.0)\\
%         Institution 8 & Prisma & syngo\_MR\_E11 & 3.0 & 2200 & 1.47 & 8 & (1.0, 1.0, 1.0)\\
%         Institution 8 & Ingenia & [5.1.7, 5.1.7.2] & 3.0 & [4.48,4.92]& [2.225, 2.45] & 8 & ([1.0, 1.2], 1.0, 1.0)\\
%         Institution 9 & Skyra & syngo\_MR\_D113C& 3.0 & 2300 & 2.98 & 9 & (1.2, 1.0, 1.0) \\
%         Institution 10 & Achieva & [3.2.1, 3.2.1.1] & 3.0& [6.36, 6.72] & [3.02, 3.14]& 8 &([1.0, 1.2], 1.0, [1.0, 1.01])\\
%         Institution 11 & Ingenia & [5.1.2, 5.1.7, 5.1.7.2] & 1.5 & [7.47, 7.90] & [3.40, 3.68] & 8 & (1.0, 1.0, 1.0) \\
%         Institution 12 & Optima MR450w & \parbox[t]{1cm}{[DV25.0\_R01\_1451.a,\\ DV25.1\_R03\_1802.a]} & 1.5 & [11.24, 11.38] & [5.0, 5.05] & 10 & (1.2, [1.0, 1.04], [1.0, 1.04]) \\
%         Institution 13 & Skyra & \parbox[t]{1cm}{[syngo\_MR\_D113C,\\ syngo\_MR\_E11]} & 3.0 & 2300 & [2.97, 2.98] & 9&(1.2, [1.0, 1.01], [1.0, 1.01]) \\
%         External Institution 1 & Prisma &syngo\_MR\_E11 & 3.0 & 2200 & 1.47 & 8 &(1.0, 1.0, 1.0)
%     \end{tabular}
%     	% }
% \end{adjustwidth}
%     \label{tab:Table1}
%     \end{table*}

    % \begin{table*}[htb]
    %     \caption{Split of MRI cases for training, validation, and testing across the different MR systems included for the 2.5D model. Avanto and Optima MR450 are 1.5 Tesla systems and the remaining 3 Tesla systems.}
    %     \begin{adjustwidth}{0cm}{}
    %     \resizebox{1\textwidth}{!}{
    %     \begin{tabular}{l|l|l|l|l|l|l}
    %         Data split & Skyra & Prisma & Ingenia & Optima MR450w & Achieva & Avanto \\\hline
    %         Training n=466 & 47 & 22 & 247 & 84 & 49 & 17\\
    %         Validation n=116 & 10 & 6 & 53 & 23 & 18 & 6\\
    %         Test (Internal)  n=60 & 5 & 3 & 30 & 12 & 8 & 2\\
    %         Test (External) n=29 & - & 29 & - & - & - & - \\
    %     \end{tabular}
    %         }
    % \end{adjustwidth}
    %     \label{tab:Table2}
    %     \end{table*}


    % \begin{table*}[htb]
    %     \caption{Performance metrics (mean +/- std.dev) for the 2.5D U-Net and 3D nnU-Net in the validation data. Shown is the model used in the experiments and the five metrics used in the white matter hyperintensity challenge for The Medical Image Computing and Computer-Assisted Intervention Society.}
    %     \begin{adjustwidth}{0cm}{}
    %     \resizebox{1\textwidth}{!}{
    %     \begin{tabular}{l|l|l|l|l|l}
    %         Model & DSC & HD95 [$mm$] & AVD [\%] & Recall & $F_{1}$ \\\hline
    %         2D U-Net & 0.70 +/- 0.14 &15.04 +/- 15.04 &37.89 +/- 33.24 &0.47 +/- 0.17 &0.59 +/- 0.13\\
    %         3D nnU-Net & 0.78 +/- 0.14 & 9.15 +/- 16.81 & 13.70 +/- 14.64 & 0.71 +/- 0.15 & 0.72 +/-0.11\\
    %     \end{tabular}
    %         }
    % \end{adjustwidth}
    %     \label{tab:Table3}
    %     \end{table*}


        % \begin{table*}[htb]
        %     \caption{Prediction metrics (lesion level) as a function of lesion size for the three models on the validation data. The values are shown as 2.5D U-Net/3D nnU-Net. The threshold set for true positive (TP) and false negatives (FN) is less than 50\% of the lesion predicted by the model, otherwise false positive (FP).
        %     }
        %     \begin{adjustwidth}{0cm}{}
        %     \resizebox{1\textwidth}{!}{
        %     \begin{tabular}{l|l|l|l|l}
        %         Lesion volume range mm$^3$ & [1, 10] & [10, 400] & [400, 1000] & [1000+ ]\\\hline
        %         Avg. Volume mm$^3$ & 8/4 & 70/54 & 624/621 & 2872/3353 \\
        %         Total & 541/1932 &2197/2317 & 108/110 & 89/87 \\
        %         Total TP & 502/864 & 1896/2216 & 107/110 & 89/87 \\
        %         Total FN & 2184/1511 & 1292/770 & 2/0 &1/1 \\
        %         Total FP & 39/1068 & 301/101 & 1/0 & 0/0 \\
        %         Recall & 0.18/0.33 & 0.57/0.65 & 0.94/0.86 & 0.96/0.89
        %     \end{tabular}
        %         }
        % \end{adjustwidth}
        %     \label{tab:Table4}
        %     \end{table*}

% \begin{table*}[htb]
%     \caption{ Performance metrics (mean +/- std.dev) for all three models in the internal test dataset. *, and \^{} indicate that the model performance is significantly better (p<0.05) compared to the 2.5D U-Net and Deep Bayesian respectively. Shown are the results from the five metrics used in the white matter hyperintensity challenge for The Medical Image Computing and Computer-Assisted Intervention Society. The values in the parenthesis are the best results from the WMH challenge.
%     }
%     \begin{adjustwidth}{0cm}{}
%     \resizebox{1\textwidth}{!}{
%     \begin{tabular}{l|l|l|l|l|l}
%          Model & DSC (0.81) & HD95 [mm] (5.63) & AVD [\%] (18.58) & Recall (0.82) & $F_{1}$ (0.79)\\\hline
%          2.5D U-Net & 0.70 +/- 0.13 & 17.02 +/- 15.97 & 45.04 +/- 51.00 & 0.50 +/- 0.18 & 0.59 +/- 0.13\\
%          3D nnU-Net & \textbf{0.78 +/- 0.10} *\^{} & \textbf{10.30 +/- 18.24} *\^{} & \textbf{16.53 +/- 15.86} *\^{} & \textbf{0.72 +/- 0.14} *\^{} & \textbf{0.71 +/- 0.10} *\^{}\\
%          Deep Bayesian & 0.63 +/- 0.15 & 17.78 +/- 12.83 & 43.24 +/- 57.92 & 0.51 +/- 0.18 & 0.56 +/- 0.14
%     \end{tabular}
%         }
% \end{adjustwidth}
%     \label{tab:Table5}
%     \end{table*}


% \begin{table*}[htb]
% \caption{Prediction metrics (lesion level) as a function of lesion size for the three models on the validation data. The values are shown as 2.5D U-Net/3D nnU-Net. The threshold set for true positive (TP) and false negatives (FN) is less than 50\% of the lesion predicted by the model, otherwise false positive (FP).}
% \begin{adjustwidth}{0cm}{}
% \resizebox{1\textwidth}{!}{
% \begin{tabular}{l|l|l|l|l}
%     Lesion volume range mm$^3$ & [1, 10] & [10, 400] & [400, 1000] & [1000+ ]\\\hline
%     Avg. Volume mm$^3$ & 8/4/3 & 72/57/67 & 625/659/663 & 2183/2101/2450 \\
%     Total & 223/963/737 &991/1024/621 & 46/45/32 & 33/33/32 \\
%     Total TP & 193/359/189 & 814/958/554 & 45/45/38 & 33/33/32 \\
%     Total FN & 826/664/834 & 464/320/724 & 0/0/7 &0/0/1\\
%     Total FP & 26/604/548 & 177/66/67 & 1/0/0 & 0/0/0 \\
%     Recall & 0.18/0.32/0.18 & 0.61/0.66/0.41 & 0.96/0.85/0.77 & 0.97/0.89/0.83
% \end{tabular}
%     }
% \end{adjustwidth}
% \label{tab:Table6}
% \end{table*}


% \begin{table*}[htb]
%     \caption{ Performance metrics (mean +/- std.dev) for all three models in the external test dataset. * and \^{} indicate that the model performance is significantly better (p<0.05) compared to the 2.5D U-Net and Deep Bayesian respectively. Shown are the results from the five metrics used in the white matter hyperintensity challenge for The Medical Image Computing and Computer-Assisted Intervention Society.
%     }
%     \begin{adjustwidth}{0cm}{}
%     \resizebox{1\textwidth}{!}{
%     \begin{tabular}{l|l|l|l|l|l}
%          Model & DSC  & HD95 [mm] & AVD [\%] & Recall & $F_{1}$\\\hline
%          2.5D U-Net & 0.54 +/- 0.19 & 22.38 +- 27.43 & 201.63 +/- 230.18 & 0.83 +/- 0.11 \^{} & \textbf{0.61 +/- 0.15} \^{}\\
%          3D nnU-Net & \textbf{0.66 +/- 0.17} *\^{} & 14.29 +/- 12.61 & 58.35 +/- 78.82 * & \textbf{0.89 +/- 0.11} \^{} & 0.56 +/- 0.12\\
%          Deep Bayesian & 0.53 +/- 0.18 & \textbf{13.41 +/- 9.45} & \textbf{48.93 +/- 41.73} * & 0.71 +/-0.16  & 0.50 +/- 0.16
%     \end{tabular}
%         }
% \end{adjustwidth}
%     \label{tab:Table7}
%     \end{table*}


% \begin{table*}[htb]
%     \caption{Prediction metrics (lesion level) as a function of lesion size for the three models on the external test data. The values are shown as 2.5D U-Net/3D nn-UNet/Deep Bayesian. The threshold set for true positive (TP) and false negatives (FN) is less than 50\% of the lesion predicted by the model, otherwise false positive (FP).
% }
%     \begin{adjustwidth}{0cm}{}
%     \resizebox{1\textwidth}{!}{
%     \begin{tabular}{l|l|l|l|l}
%         Lesion volume range mm$^3$ & [1, 10] & [10, 400] & [400, 1000] & [1000+ ]\\\hline
%         Avg. Volume mm$^3$ & 8/4/3 & 71/53/77 & 640/601/582 & 3704/2694/2436 \\
%         Total & 33/391/380 &610/523/283 & 17/16/14 & 19/18/16 \\
%         Total TP & 14/14/4 & 351/326/203 & 16/16/14 & 18/18/16 \\
%         Total FN & 26/26/36 & 69/94/217 & 0/0/2 &0/0/2\\
%         Total FP & 19/377/376 & 259/197/80 & 1/0/0 & 1/0/0 \\
%         Recall & 0.31/0.32/0.11 & 0.78/0.67/0.45 & 0.98/0.89/0.75 & 0.98/0.88/0.73
%     \end{tabular}
%         }
%     \end{adjustwidth}
%     \label{tab:Table8}
%     \end{table*}
